Toward Expressive Singing Voice Correction: On Perceptual Validity of Evaluation Metrics for Vocal Melody Extraction

Singing voice correction (SVC) is an appealing application for amateur singers. Commercial products automate SVC by snapping pitch contours to equal-tempered scales, which could lead to deadpan modifications. Together with the neglect of rhythmic errors, extensive manual corrections are still necessary. In this paper, we present a streamlined system to automate expressive SVC for both pitch and rhythmic errors. Particularly, we extend a previous work by integrating advanced techniques for singing voice separation (SVS) and vocal melody extraction. SVC is achieved by temporally aligning the source-target pair, followed by replacing pitch and rhythm of the source with those of the target. We evaluate the framework by a comparative study for melody extraction which involves both subjective and objective evaluations, whereby we investigate perceptual validity of the standard metrics through the lens of SVC. The results suggest that the high pitch accuracy obtained by the metrics does not signify good perceptual scores.

==> prgs/related.tex <==
\section{Related Works}\label{sec:related}
Commercial products such as Antares \textit{Auto-Tune}~\cite{autotune} and Celemony \textit{Melodyne}~\cite{melodyne} snap a pitch contour to nearest notes defined by a reference, or a target, which can be either a musical scale or a known score.
Guslar~\cite{azarov2014guslar} processes the reference with smoothing and vibrato in order to improve naturalness of the target melody.
A data-driven~\cite{wager2020deep} approach is proposed to achieve pitch correction by predicting original singing using its artificially pitch-shifted version.
The application of singing voice alignment for SVC~\cite{luo2018singing} exploits pitch contours extracted from real singing as the target, whereby expressive parameters are readily available.
Unlike the deep learning based method~\cite{wager2020deep}, the approach can handle sources with large pitch errors, as the source pitch contours are directly replaced with those of the targets.
Automatic rendering of target singing is also explored in a previous work~\cite{yong2018}.
Though the method bears a resemblance to the proposed framework, it focuses on singing expression transfer instead of pitch correction and thereby does not rectify pitch contours that are much deviated.
Moreover, they only attend to singing voice without background music, and do not analyze impacts of different melody extractors.

% We extend the approach~\cite{luo2018singing} by integrating SVS which enhances its applicability, and by enabling rhythmic correction.
% Furthermore, we present a comparative study of SOTA melody extractors, perform correlation analysis between standard metrics and subjective criteria, and highlight the
